PHiLIP on the HiL: Automated Multi-platform OS Testing with External Reference Devices

Developing an operating system (OS) for low-end embedded devices requires continuous adaptation to new hardware architectures and components, while serviceability of features needs to be assured for each individual platform under tight resource constraints. It is challenging to design a versatile and accurate heterogeneous test environment that is agile enough to cover a continuous evolution of the code base and platforms. This mission is even morehallenging when organized in an agile open-source community process with many contributors such as for the RIOT OS. Hardware in the Loop (HiL) testing and Continuous Integration (CI) are automatable approaches to verify functionality, prevent regressions, and improve the overall quality at development speed in large community projects. In this paper, we present PHiLIP (Primitive Hardware in the Loop Integration Product), an open-source external reference device together with tools that validate the system software while it controls hardware and interprets physical signals. Instead of focusing on a specific test setting, PHiLIP takes the approach of a tool-assisted agile HiL test process, designed for continuous evolution and deployment cycles. We explain its design, describe how it supports HiL tests, evaluate performance metrics, and report on practical experiences of employing PHiLIP in an automated CI test infrastructure. Our initial deployment comprises 22 unique platforms, each of which executes 98 peripheral tests every night. PHiLIP allows for easy extension of low-cost, adaptive testing infrastructures but serves testing techniques and tools to a much wider range of applications.

==> Makefile <==
DOC=main
FINALDOC=paper

pdf:
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex

all:
	pdflatex $(DOC).tex
	bibtex $(DOC)
	pdflatex $(DOC).tex
	pdflatex $(DOC).tex

clean:
	rm -f $(DOC).blg $(DOC).bbl $(DOC).aux $(DOC).log $(DOC).pdf \
	      $(DOC).synctex.gz $(DOC).out $(FINALDOC).zip $(FINALDOC).pdf

texdiff:
	latexdiff-vc --allow-spaces --append-safecmd="philip,philippal,ac,acp,mmm,xspace,eurosym" -t CFONT --git --flatten -r submission main.tex
	pdflatex main-diffsubmission.tex
	pdflatex main-diffsubmission.tex

zipadedoo: all
	cp main.pdf $(FINALDOC).pdf 
	zip $(FINALDOC).zip *.tex Makefile *.bbl -r figs


==> conclusion.tex <==
\section{Conclusion and Outlook}
\label{sec:conclusion}

In this paper, we presented a concept and implementation for performing hardware-in-the-loop tests for low-end IoT devices.
Part of the solution are two crucial components:
\philip, an open-source external reference device,
and a process that simplifies verification of peripheral behavior on different embedded hardware platforms.

The testing tool and process is built to be accessible to typical embedded developers opening it for further extensions and maintenance in an agile way.
Our approach is scalable and thus considers a plethora of IoT hardware, one of the core challenges in IoT scenarios.
We reported on our deployment that helps improving the quality of a popular IoT operating system.
It currently hosts 20 unique DUTs, representing, to the best of our knowledge, the widest variety of supported boards amongst comparable operating systems.
% Maybe we could say we have the widest variety of supported boards (20), while others usually only have 3 to 5 different boards?
Based on practical experience, we showed that our concepts are ready for production use, providing insights for the IoT testing ecosystem in general.
Additionally, we highlighted how the automation of integral parts of the testing process adds benefits for daily development work.

Future work could reduce the overhead of the test firmware on the DUT, by leveraging a more efficient serialization of commands and responses.
The access control provided by the \mmm could also be further compressed by using bit-fields instead of bytes.
Power consumption regression tests can be implemented by using the additional hardware provided by the \bph.
Improving the reliability of flashing DUTs could benefit DUT availability.
The system can also be used to qualify peripherals of emulators such as Renode or QEMU by comparing emulated results with results from the HiL tests.
% Feature support sheets
